Hyper-parameter Tuning under a Budget Constraint

We study a budgeted hyper-parameter tuning problem, where we optimize the tuning result under a hard resource constraint. We propose to solve it as a sequential decision making problem, such that we can use the partial training progress of configurations to dynamically allocate the remaining budget. Our algorithm combines a Bayesian belief model which estimates the future performance of configurations, with an action-value function which balances exploration-exploitation tradeoff, to optimize the final output. It automatically adapts the tuning behaviors to different constraints, which is useful in practice. Experiment results demonstrate superior performance over existing algorithms, including the-state-of-the-art one, on real-world tuning tasks across a range of different budgets.

==> property.tex <==
%!TEX root = main.tex
\section{Behavior}
First, we introduce the notations.
\begin{table}[htbp]
\hspace*{-1cm} 
%\begin{adjustbox}{width=1.2\textwidth}
\centering
\begin{tabular}{c|l}
\hline
notation & \multicolumn{1}{c}{ in hyperparameter tuning}  \\
\hline
$\nu^\m_{|n}$ & r.v. of the achievable performance of configuration $\m$ \\ \hline
$\theta^\m_{|n}$ & expectation of the achievable performance of configuration $\m$ \\ \hline
$\mathpzc{k}_n^*$ & optimal configuration \\ \hline
%$\tau_n^*$ & epoch that achieves the optimal performance \\ \hline
$\nu^*_{|n}, \theta^*_{|n}$ & the optimal performance of $\mathpzc{k}_n^*$ at epoch $\tau_n^*$\\ \hline
\end{tabular}
%\end{adjustbox}
\caption{Notations of action-value function} \label{table:notation2}
\end{table}

\begin{align}
 & \mQ^{(1)}_n[a]  =  \ProbOpr{E}_{n}\left[\min \{ \nu^a_{|n},  \min_{\m \neq a }\theta_{|n}^\m \} \right]  \notag \\
& = \begin{cases}
     \expect{n}{\min \{ \nu^a_{|n},  \theta_{|n}^{\mathpzc{k}_n^*} \}\}}, & \text{ when } a \neq \mathpzc{k}_n^*, \\
    \expect{n}{\min \{ \nu^{\mathpzc{k}_n^*}_{|n},  \theta_{|n}^{\mathrm{2nd}} \}},     &\text{ when } a = \mathpzc{k}_n^*,
\end{cases}
\label{eq:acq1}
\end{align}

\begin{align}
\mQ^{(1)}_n & = \expect{\nu}{\min\{\nu, \theta\}} = \theta - \std{}{\nu} \big(s\Phi(s) +  \phi(s)  \big) \notag \\
\mQ^{(2)}_n & = \expect{\nu_1, \nu_2}{\min\{\nu_1, \nu_2\}}  = \expect{}{\nu_1} - \sigma[\nu_1 \! - \! \nu_2]\big(r\Phi(r) +  \phi(r)  \big) \label{eq:acq2_compute}
\end{align}



\begin{lemma} When $B \to \infty$, all configurations get selected infinitely often.
\end{lemma}

